Orthogonal Time Frequency Space for Integrated Sensing and Communication: A Survey

Sixth-generation (6G) wireless communication systems, as stated in the European 6G flagship project Hexa-X, are anticipated to feature the integration of intelligence, communication, sensing, positioning, and computation. An important aspect of this integration is integrated sensing and communication (ISAC), in which the same waveform is used for both systems both sensing and communication, to address the challenge of spectrum scarcity. Recently, the orthogonal time frequency space (OTFS) waveform has been proposed to address OFDM's limitations due to the high Doppler spread in some future wireless communication systems. In this paper, we review existing OTFS waveforms for ISAC systems and provide some insights into future research. Firstly, we introduce the basic principles and a system model of OTFS and provide a foundational understanding of this innovative technology's core concepts and architecture. Subsequently, we present an overview of OTFS-based ISAC system frameworks. We provide a comprehensive review of recent research developments and the current state of the art in the field of OTFS-assisted ISAC systems to gain a thorough understanding of the current landscape and advancements. Furthermore, we perform a thorough comparison between OTFS-enabled ISAC operations and traditional OFDM, highlighting the distinctive advantages of OTFS, especially in high Doppler spread scenarios. Subsequently, we address the primary challenges facing OTFS-based ISAC systems, identifying potential limitations and drawbacks. Then, finally, we suggest future research directions, aiming to inspire further innovation in the 6G wireless communication landscape.

==> bibitemref.tex <==

\begin{thebibliography}{1}

\bibitem{otfs_basic0}
R. Hadani, S. Rakib, M. Tsatsanis, A. Monk, A. J. Goldsmith, A. F. Molisch, and R. Calderbank,
``Orthogonal Time Frequency Space Modulation,''
\emph{Wireless Communications and Networking Conference (WCNC)}, San Francisco, CA, USA, March 2017.

\bibitem{6gbeyond}
Ashu Taneja, Adi Alhudhaif, Shtwai Alsubai, and Abdullah Alqahtani,
``A Novel Multiple Access Scheme for 6G Assisted Massive Machine Type Communication,''
\emph{IEEE Access}, vol. 10, pp. 117638-117645, November 2022.
\bibitem{5gbasic0}
Jeffrey G. Andrews, Stefano Buzzi, Wan Choi, Stephen V. Hanly, Angel Lozano, Anthony C. K. Soong, and Jianzhong Charlie Zhang,
``What Will 5G Be?''
\emph{IEEE Journal on Selected Areas in Communications}, vol. 32, no. 6, pp. 1065-1082, June 2014.
\bibitem{5gbasic}
Walid Saad, Mehdi Bennis, and Mingzhe Chen,
``A Vision of 6G Wireless Systems: Applications, Trends, Technologies, and Open Research Problems,''
\emph{IEEE Network}, vol. 34, no. 3, pp. 134-142, October 2020.

\bibitem{5gbasic1}
Erik Dahlman, Gunnar Mildh, Stefan Parkvall, Janne Peisa, Joachim Sachs, Yngve Selén, and Johan Sköld,
``5G Wireless Access: Requirements and Realization,''
\emph{IEEE Communications Magazine}, vol. 52, no. 12, pp. 42-47, December 2014.
\bibitem{5gmmwave1}
Wei Hong, Zhi Hao Jiang, Chao Yu, Debin Hou, Haiming Wang, Chong Guo, Yun Hu, Le Kuai, Yingrui Yu, Zhengbo Jiang, Zhe Chen, Jixin Chen, Zhiqiang Yu, Jianfeng Zhai, Nianzu Zhang, Ling Tian, Fan Wu, Guangqi Yang, Zhang-Cheng Hao, and Jian Yi Zhou,
``The Role of Millimeter-Wave Technologies in 5G/6G Wireless Communications,''
\emph{IEEE Journal of Microwaves}, vol. 1, no. 1, pp. 101-122, January 2021.

\bibitem{5gmmwave2}
Mousa Abdollahvand, Eduardo Martinez-de-Rioja, Jose A. Encinar, and Kanishka Katoch,
``Dual-Band Single-Layer Frequency Selective Surface for Millimeter-Wave 5G Applications,''
in \emph{European Conference on Antennas and Propagation (EuCAP)}, Florence, Italy, March 2023.


\bibitem{5gmmwave3}
Abdul Jabbar, Muhammad Ali Jamshed, Mahmoud A. Shawky, Qammer H. Abbasi, Muhammad Ali Imran, and Masood Ur Rehman,
``Multi-Gigabit Millimeter-Wave Industrial Communication: A Solution for Industry 4.0 and Beyond,''
in \emph{IEEE Global Communications Conference}, Rio de Janeiro, Brazil, December 2022.

\bibitem{5gmmwave4}
Joshua Onolemhemhen, Sadiq Thomas, Omotayo Oshiga, Tologon Karataev, Opeyemi Osanaiye, and Oluseun Oyeleke,
``A Review of 5G Millimeter Waves and Enabling Technologies for IoT,''
in \emph{International Conference on Multidisciplinary Engineering and Applied Science (ICMEAS)}, Abuja, Nigeria.

\bibitem{5gmmwave5}
Zu-Kai Weng, Atsushi Kanno, Pham Tien Dat, Keizo Inagaki, Kosuke Tanabe, Eisaku Sasaki, Thomas Kürner, Bo Kum Jung, and Tetsuya Kawanishi,
``Millimeter-Wave and Terahertz Fixed Wireless Link Budget Evaluation for Extreme Weather Conditions,''
\emph{IEEE Access}, vol. 9, pp. 163476-163491, December 2021.

\bibitem{UDN1}
Radostina Petkova, Antoni Ivanov, and Vladimir Poulkov,
``Challenges in Implementing Ultra-Dense Scenarios in 5G Networks,''
in \emph{Joint International Conference on Digital Arts, Media and Technology with ECTI Northern Section Conference on Electrical, Electronics, Computer and Telecommunications Engineering (ECTI DAMT \& NCON)}, Pattaya, Thailand, May 2020.

\bibitem{UDN2}
Qirui Liu, Rongke Liu, Zijie Wang, and Yifan Zhang,
``Simulation and Analysis of Device Positioning in 5G Ultra-Dense Network,''
in \emph{International Wireless Communications & Mobile Computing Conference (IWCMC)}, Tangier, Morocco, June 2019.

\bibitem{UDN3}
Xiaohu Ge, Song Tu, Guoqiang Mao, Cheng-Xiang Wang, and Tao Han,
``5G Ultra-Dense Cellular Networks,''
\emph{IEEE Wireless Communications}, vol. 23, no. 1, pp. 72-79, February 2016.

\bibitem{UDN4}
Mahmoud Kamel, Walaa Hamouda, and Amr Youssef,
``Ultra-Dense Networks: A Survey,''
\emph{IEEE Communications Surveys \& Tutorials}, vol. 18, no. 4, pp. 2522-2545, May 2016.

\bibitem{UDN5}
Garima Chopra, Rakesh Kumar Jha, and Sanjeev Jain,
``Security Issues in Ultra Dense Network for 5G Scenario,''
in \emph{International Conference on Communication Systems \& Networks (COMSNETS)}, Bengaluru, India, January 2018.
\bibitem{UDN6}
Debashis Dev Misra and Kandarpa Kumar Sarma,
``Cooperative Routing Mechanism in the 5G Ultra Dense Network,''
in \emph{International Conference on Signal Processing and Integrated Networks (SPIN)}, Noida, India, February 2018.

\bibitem{UDN7}
Younghoon Jo, Hojin Kim, Jaechan Lim, and Daehyoung Hong,
``Self-Optimization of Coverage and System Throughput in 5G Heterogeneous Ultra-Dense Networks,''
\emph{IEEE Wireless Communications Letters}, vol. 9, no. 3, pp. 285-288, November 2020.

\bibitem{5gmmimo1}
Zizheng Wang, Dake Shi, and Haotian Wu,
``The Role of Massive MIMO and Intelligent Reflecting Surface in 5G/6G Networks,''
in \emph{International Conference on Wireless Communications and Smart Grid (ICWCSG)}, Hangzhou, China, August 2021.

\bibitem{5gmmimo2}
Sunita Dhalbisoi, Ashima Rout, Ramesh Kumar Sahoo, and Srinivas Sethi,
``A Comparative Analysis On 5G Cell Free Massive MIMO In Next Generation Networking Environment,''
in \emph{International Conference on Intelligent Controller and Computing for Smart Power (ICICCSP)}, Hyderabad, India, July 2022.

\bibitem{5gmmimo3}
Md. Yeakub Ali, Tamanna Hossain, and Md. Munjure Mowla,
``A Trade-off between Energy and Spectral Efficiency in Massive MIMO 5G System,''
in \emph{International Conference on Electrical, Computer \& Telecommunication Engineering (ICECTE)}, Rajshahi, Bangladesh, December 2019.


\bibitem{5gmmimo4}
Mithra Venkatesan, Anju Kulkarni, Radhika Menon, and Shashikant Prasad,
``Interference Mitigation Approach using Massive MIMO towards 5G networks,''
in \emph{Asian Conference on Innovation in Technology (ASIANCON)}, Ravet, India, August 2022.

\bibitem{5g001}
Afif Osseiran, Federico Boccardi, Volker Braun, Katsutoshi Kusume, Patrick Marsch, Michal Maternia, Olav Queseth, Malte Schellmann, Hans Schotten, Hidekazu Taoka, Hugo Tullberg, Mikko A. Uusitalo, Bogdan Timus, and Mikael Fallgren,
``Scenarios for 5G mobile and wireless communications: the vision of the METIS project,''
\emph{IEEE Communications Magazine}, vol. 52, no. 5, pp. 26-35, May 2014.
\bibitem{5g002}
Ronald Beaubrun,
``Technical Challenges and Categorization of 5G Mobile Services,''
in \emph{Thirteenth International Conference on Ubiquitous and Future Networks (ICUFN)}, Barcelona, Spain, July 2022.

\bibitem{HST1}
Xiaoyin Zhao, Zhijun Li, Chunlei Hu, Jia Hou, and Weiliang Xie,
``Solutions of 5G RAN on High-Speed Train: Proposed for 5G RAN system equipped directly onto the high-speed train,''
in \emph{International Conference on Communication Engineering and Technology (ICCET)}, Shanghai, China, February 2022.

\bibitem{HST2}
Juho Park, Junghoon Lee, JunHwan Lee, and Moon-Sik Lee,
``Enabling 5G Techniques to Support HD Video Streaming to High-Speed Train Users,''
In \emph{International Conference on Information and Communication Technology Convergence (ICTC)}, Jeju, Korea (South), October 2020.

\bibitem{HST3}
Bo Ai, Ke Guan, Markus Rupp, Thomas Kurner, Xiang Cheng, Xue-Feng Yin, Qi Wang, Guo-Yu Ma, Yan Li, Lei Xiong, and Jian-Wen Ding,
``Future railway services-oriented mobile communications network,''
\emph{IEEE Communications Magazine}, vol. 53, no. 10, pp. 78-85, October 2015.


\bibitem{HST4}
Nobuhide Nonaka, Kazushi Muraoka, Tatsuki Okuyama, Satoshi Suyama, Yukihiko Okumura, Takahiro Asai, and Yoshihiro Matsumura,
``28 GHz-Band Experimental Trial at 283 km/h Using the Shinkansen for 5G Evolution,''
in \emph{IEEE 91st Vehicular Technology Conference (VTC2020-Spring)}, Antwerp, Belgium, May 2020.



\bibitem{HST}
Ke Guan, Bo Ai, Bile Peng, Danping He, Guangkai Li, Jingya Yang, Zhangdui Zhong, and Thomas Kürner,
``Towards Realistic High-Speed Train Channels at 5G Millimeter-Wave Band—Part II: Case Study for Paradigm Implementation,''
\emph{IEEE Transactions on Vehicular Technology}, vol. 67, no. 10, pp. 9129-9144, August 2018.

\bibitem{HST5}
Jiayi Zhang, Hongyang Du, Peng Zhang, Julian Cheng, and Liang Yang,
``Performance Analysis of 5G Mobile Relay Systems for High-Speed Trains,''
\emph{IEEE Journal on Selected Areas in Communications}, vol. 38, no. 12, pp. 2760-2772, June 2020.

\bibitem{HST6}
Lei Ma, Ke Guan, Dong Yan, Danping He, Bo Ai, Junhyeong Kim, and Heesang Chung,
``Characterization for High-Speed Railway Channel enabling Smart Rail Mobility at 22.6 GHz,''
in \emph{IEEE Wireless Communications and Networking Conference (WCNC)}, Seoul, Korea (South), May 2020.

\bibitem{HST7}
Berna Bulut,
``5G NR C-V2V for High Speed Train Safety Applications,''
in \emph{Signal Processing and Communications Applications Conference (SIU)}, Gaziantep, Turkey, October 2020.


\bibitem{HST8}
Xiaoyin Zhao, Zhijun Li, Chunlei Hu, Jia Hou, and Weiliang Xie,
``Solutions of 5G RAN on High-Speed Train: Proposed for 5G RAN system equipped directly onto the high-speed train,''
in \emph{International Conference on Communication Engineering and Technology (ICCET)}, Shanghai, China, February 2022.

\bibitem{v2x1}
Md. Sazzad Hossen, Min-Suk Bang, Youngil Park, and Ki-Doo Kim,
``Performance analysis of an OFDM-based method for V2X communication,''
in \emph{International Conference on Ubiquitous and Future Networks (ICUFN)}, Shanghai, China, February 2014.

\bibitem{v2x2}
Haibin Chen, Rongqing Zhang, Wenjun Zhai, Xiaoli Liang, and Guojuan Song,
``Interference-free pilot design and channel estimation using ZCZ sequences for MIMO-OFDM-based C-V2X communications,''
\emph{China Communications}, vol. 15, no. 7, pp. 47-54, July 2018.

\bibitem{v2x3}
Erik G. Ström,
``On 20 MHz channel spacing for V2X communication based on 802.11 OFDM,''
in \emph{Annual Conference of the IEEE Industrial Electronics Society (IECON 2013)}, Vienna, Austria, November 2013.

\bibitem{v2x4}
Shenglin Xu, Hu Liu, Sheng Zhang, and Qingqing Liu,
``A joint detection algorithm of integer frequency offset estimation and cell ID based on 5G-NR-V2X,''
in \emph{International Conference on Advanced Electronic Materials, Computers and Software Engineering (AEMCSE)}, Wuhan, China, April 2022.

\bibitem{uavofdm1}
He Jian and Zhang Yue-tong,
``Impact of Doppler on High-Speed UAV OFDM System,''
In \emph{International Conference on Communication Software and Networks (ICCSN 2009)}, Chengdu, China, February 2009.

\bibitem{uavofdm2}
Xiaopeng Tan, Shaojing Su, Xiaojun Guo, and Xiaoyong Sun,
``Application of MIMO-OFDM Technology in UAV Communication Network,''
in \emph{2nd World Symposium on Artificial Intelligence (WSAI)}, Guangzhou, China, June 2020.

\bibitem{ofdmici}
Nilesh Kumar Jadav,
``A Survey on OFDM Interference Challenge to improve its BER,''
in \emph{Second International Conference on Electronics, Communication and Aerospace Technology (ICECA)}, Coimbatore, India, March 2018.

\bibitem{ofdmici1}
Hamid Nourollahi and Saeed Ghazi Maghrebi,
``Evaluation of cyclic prefix length in OFDM system based for Rayleigh fading channels under different modulation schemes,''
in \emph{IEEE Symposium on Computers and Communications (ISCC 2017)}, Heraklion, Greece, July 2017.
\bibitem{ofdmici2}
Yasir Rahmatallah and Seshadri Mohan,
``Peak-To-Average Power Ratio Reduction in OFDM Systems: A Survey And Taxonomy,''
\emph{IEEE Communications Surveys \& Tutorials}, vol. 15, no. 4, pp. 1567-1592, March 2013.


\bibitem{ofdmpar}
U. B. Mahadevaswamy and M. N. Geetha,
``A comparative survey on PAPR reduction in OFDM signal,''
in \emph{International Conference on Electrical, Electronics, Communication, Computer and Optimization Techniques (ICEECCOT)}, 
Mysuru, India, December 2016.
\bibitem{ofdmsynch}
Pushpa Kotipalli,
``Preamble-based joint frame and frequency synchronization for OFDM — WMAN systems,''
in \emph{11th International Conference on Hybrid Intelligent Systems (HIS)}, 
Melacca, Malaysia, December 2011.

\bibitem{otfs_basic1}
Saif Khan Mohammed,
``Derivation of OTFS Modulation From First Principles,''
\emph{IEEE Transactions on Vehicular Technology}, 
vol. 70, no. 8, pp. 7619-7636, March 2021.
\bibitem{ofdma1}
L. Lu, G. Y. Li, A. L. Swindlehurst, A. Ashikhmin, and R. Zhang, ``An Overview of Massive MIMO: Benefits and Challenges,'' \emph{IEEE Journal of Selected Topics in Signal Processing}, vol. 8, no. 5, pp. 742-758, April 2014.

\bibitem{ofdma2}
T. M. Schmidl and D. C. Cox, ``Robust frequency and timing synchronization for OFDM,'' \emph{IEEE Transactions on Communications}, vol. 45, no. 12, pp. 1613-1621, December 1997.

\bibitem{ofdma3}
A. J. Paulraj, D. A. Gore, R. U. Nabar, and H. Bolcskei, ``An overview of MIMO communications - a key to gigabit wireless,'' \emph{Proceedings of the IEEE}, vol. 92, no. 2, pp. 198-218, February 2004.
\bibitem{ofdma4}
O. Edfors, M. Sandell, J.-J. van de Beek, S. K. Wilson, and P. O. Borjesson, ``OFDM channel estimation by singular value decomposition,'' \emph{IEEE Transactions on Communications}, vol. 46, no. 7, pp. 931-939, August 1998.
\bibitem{ofdma5}
L. Cimini, ``Analysis and Simulation of a Digital Mobile Channel Using Orthogonal Frequency Division Multiplexing," \emph{IEEE Transactions on Communications}, vol. 33, no. 7, pp. 665-675, July 1985.

\bibitem{ICI_in_ISAC2}
G. Hakobyan and B. Yang,  ``A Novel Intercarrier-Interference Free Signal Processing Scheme for OFDM Radar," \emph{IEEE Transactions on Vehicular Technology}, vol. 67, no. 6, pp. 5158-5167, July 2018.

\bibitem{ICI_in_ISAC}
M. F. Keskin, H. Wymeersch, and V. Koivunen,  ``MIMO-OFDM Joint Radar-Communications: Is ICI Friend or Foe?," \emph{IEEE Journal of Selected Topics in Signal Processing}, vol. 15, no. 6, pp. 1393-1408, September 2021.

\bibitem{ICI_in_ISAC3}
J. Lim, S. Kim, and D. Shin,  ``Two-Step Doppler Estimation Based on Intercarrier Interference Mitigation for OFDM Radar," \emph{IEEE Antennas and Wireless Propagation Letters}, vol. 14, pp. 1726-1729, April 2015.

\bibitem{intro_2_channel}
Y. Li, S. Wang, J. Jin, W. Xiang, and H. Long, ``Doppler Shift Estimation Based Channel Estimation for Orthogonal Time Frequency Space System,'' in \emph{IEEE 94th Vehicular Technology Conference (VTC2021-Fall)}, Norman, OK, USA, September 2021, pp. 1-6.

\bibitem{otfs_intro0}
Y. Liang, L. Li, P. Fan, and Y. Guan, ``Doppler Resilient Orthogonal Time-Frequency Space (OTFS) Systems Based on Index Modulation,'' in \emph{IEEE 91st Vehicular Technology Conference (VTC2020-Spring)}, Antwerp, Belgium, May 2020.


\bibitem{ofdma2}
T. M. Schmidl and D. C. Cox, ``Robust frequency and timing synchronization for OFDM,'' \emph{IEEE Transactions on Communications}, vol. 45, no. 12, pp. 1613-1621, December 1997.

\bibitem{otfs_intro02}
R. Hadani, S. Rakib, A. F. Molisch, C. Ibars, A. Monk, M. Tsatsanis, J. Delfeld, A. Goldsmith, and R. Calderbank, ``Orthogonal Time Frequency Space (OTFS) modulation for millimeter-wave communications systems,'' in \emph{IEEE MTT-S International Microwave Symposium (IMS)}, Honolulu, HI, USA, June 2017.
\bibitem{otfs_intro1}
Wenqian Shen, Linglong Dai, Jianping An, Pingzhi Fan, and Robert W. Heath, ``Channel Estimation for Orthogonal Time Frequency Space (OTFS) Massive MIMO,'' \emph{IEEE Transactions on Signal Processing}, vol. 67, no. 16, pp. 4204-4217, May 2019.

\bibitem{otfs_intro2}
Lorenzo Gaudio, Mari Kobayashi, Giuseppe Caire, and Giulio Colavolpe, ``On the Effectiveness of OTFS for Joint Radar Parameter Estimation and Communication,'' \emph{IEEE Transactions on Wireless Communications}, vol. 19, no. 9, pp. 5951-5965, June 2020.

\bibitem{otfs_intro3}
Shashank Tiwari, Suvra Sekhar Das, and Vivek Rangamgari, ``Low complexity LMMSE Receiver for OTFS,'' \emph{IEEE Communications Letters}, vol. 23, no. 12, pp. 2205-2209, October 2019.

\bibitem{otfs_intro4}
G. D. Surabhi and A. Chockalingam, ``Low-Complexity Linear Equalization for OTFS Modulation," \emph{IEEE Communications Letters}, vol. 24, no. 2, pp. 330-334, November 2020.
\bibitem{otfs_intro5}
P. Raviteja, Yi Hong, Emanuele Viterbo, and Ezio Biglieri, ``Effective Diversity of OTFS Modulation," \emph{IEEE Wireless Communications Letters}, vol. 9, no. 2, pp. 249-253, November 2020.

\bibitem{intro_2_channel4}
P. Raviteja, Khoa T. Phan, Yi Hong, and Emanuele Viterbo, ``Embedded Delay-Doppler Channel Estimation for Orthogonal Time Frequency Space Modulation,'' in \emph{IEEE 88th Vehicular Technology Conference (VTC-Fall)}, Chicago, IL, USA, August 2018.

\bibitem{intro_2_channel5}
Xiang Li, Weijie Yuan, and Zhongjie Li, ``Hybrid Message Passing Detection for OTFS Modulation,'' in \emph{IEEE Wireless Communications and Networking Conference (WCNC)}, Glasgow, United Kingdom, March 2023.
\bibitem{intro_2_channel6}
Zongming Yuan, Meng Tang, Jianhua Chen, Taibin Fang, Hao Wang, and Jinhong Yuan, ``Low Complexity Parallel Symbol Detection for OTFS Modulation,'' \emph{IEEE Transactions on Vehicular Technology}, vol. 72, no. 4, pp. 4904-4918, December 2023.
\bibitem{intro_2_channel7}
Wei Liu, Yajie Ding, Chuan Li, and Lajos Hanzo, ``Optimal Low-Complexity Orthogonal Block Based Detection of OTFS for Low-Dispersion Channels,'' \emph{IEEE Transactions on Vehicular Technology}, vol. 72, no. 4, pp. 5419-5423, November 2023.

\bibitem{otfs1111}
Shuangyang Li, Weijie Yuan, Zhiqiang Wei, and Jinhong Yuan, ``Cross Domain Iterative Detection for Orthogonal Time Frequency Space Modulation,'' \emph{IEEE Transactions on Wireless Communications}, vol. 21, no. 4, pp. 2227-2242, September 2022.

\bibitem{otfs1112}
Zhengdao Yuan, Fei Liu, Weijie Yuan, Qinghua Guo, Zhongyong Wang, and Jinhong Yuan, ``Iterative Detection for Orthogonal Time Frequency Space Modulation With Unitary Approximate Message Passing,'' \emph{IEEE Transactions on Wireless Communications}, vol. 21, no. 2, pp. 714-725, February 2022.

\bibitem{10012849}
Xiangnan Xu, Ping Yang, Bo Zhang, Yue Xiao, and Shaoqian Li, ``An Improved PAPR Reduction Method Based on Imperialist Competition Algorithm for OTFS System,'' in \emph{2022 IEEE 96th Vehicular Technology Conference (VTC2022-Fall)}, London, United Kingdom, September 2022.


\bibitem{intro_3_spectral}
Venkatesh Khammammetti and Saif Khan Mohammed, ``Spectral Efficiency of OTFS Based Orthogonal Multiple Access With Rectangular Pulses,'' \emph{IEEE Transactions on Vehicular Technology}, vol. 71, no. 12, pp. 12989-13006, August 2022.

\bibitem{intro_3_spectral2}
Tiejun Wang and J.G. Proakis and E. Masry and J.R. Zeidler, ``Performance degradation of OFDM systems due to Doppler spreading,'' \emph{IEEE Transactions on Wireless Communications}, vol. 5, no. 6, pp. 1422-1432, June 2006.

\bibitem{intro_3_spectral3}
P. Bello, ``Characterization of Randomly Time-Variant Linear Channels,'' \emph{IEEE Transactions on Communications Systems}, vol. 11, no. 4, pp. 360-393, December 1963.

\bibitem{intro1}
V. Khammammetti and S. Khan, ``OTFS-Based Multiple-Access in High Doppler and Delay Spread Wireless Channels,'' \emph{IEEE Wireless Communications Letters}, vol. 8, no. 2, pp. 528-531, October 2019.

\bibitem{intro_2_channel1}
H. Zhang, J. Li, T. Zhang, and X. Zhu, ``An Efficient Channel Estimation Scheme for Short Frame OTFS Using Impulse-Train Pilots,'' in \emph{IEEE Global Communications Conference}, Rio de Janeiro, Brazil, December 2022.

\bibitem{intro_2_channel2}
L. Li, Y. Liang, P. Fan, and Y. Guan, ``Low Complexity Detection Algorithms for OTFS under Rapidly Time-Varying Channel,'' in \emph{IEEE 89th Vehicular Technology Conference (VTC2019-Spring)}, Kuala Lumpur, Malaysia, May 2019.

\bibitem{intro_2_channel3}
P. Raviteja, K. T. Phan, and Y. Hong, ``Embedded Pilot-Aided Channel Estimation for OTFS in Delay–Doppler Channels,'' \emph{IEEE Transactions on Vehicular Technology}, vol. 68, no. 5, pp. 4906-4917, March 2019.


\bibitem{ICI_in_ISAC1}
F. Liu, C. Masouros, A. P. Petropulu, H. Griffiths, and L. Hanzo, ``Joint Radar and Communication Design: Applications, State-of-the-Art, and the Road Ahead,'' \emph{IEEE Transactions on Communications}, vol. 68, no. 6, pp. 3834-3862, February 2020.

\bibitem{ICI_in_ISAC4}
Y. Ge, W. Zhang, F. Gao, and H. Minn, ``Angle-Domain Approach for Parameter Estimation in High-Mobility OFDM With Fully/Partly Calibrated Massive ULA," \emph{IEEE Transactions on Wireless Communications}, vol. 18, no. 1, pp. 591-607, December 2019.
\bibitem{ICI_in_ISAC5}
R. F. Tigrek, W. J. A. De Heij, and P. Van Genderen, ``OFDM Signals as the Radar Waveform to Solve Doppler Ambiguity,'' \emph{IEEE Transactions on Aerospace and Electronic Systems}, vol. 48, no. 1, pp. 130-143, January 2012.

\bibitem{ICI_in_ISAC6}
M. F. Keskin, C. Marcus, O. Eriksson, H. Wymeersch, and V. Koivunen, ``On the Impact of Phase Noise on Monostatic Sensing in OFDM ISAC Systems,'' in \emph{IEEE Radar Conference (RadarConf23)}, San Antonio, TX, USA, May 2023.

\bibitem{intro2}
R. Hadani, S. Rakib, M. Tsatsanis, A. Monk, A. J. Goldsmith, A. F. Molisch, and R. Calderbank, ``Orthogonal Time Frequency Space Modulation,'' in \emph{IEEE Wireless Communications and Networking Conference (WCNC)}, San Francisco, CA, USA, March 2017.

\bibitem{intro3}
K. R. Murali and A. Chockalingam, ``On OTFS Modulation for High-Doppler Fading Channels,'' in \emph{Information Theory and Applications Workshop (ITA)}, San Diego, CA, USA, February 2018.

\bibitem{ofdm1}
S. He, Q. Zhang, and J. Qin, ``Pilot Pattern Design for Two-Dimensional OFDM Modulations in Time-Varying Frequency-Selective Fading Channels,'' \emph{IEEE Transactions on Wireless Communications}, vol. 21, no. 2, pp. 1335-1346, February 2022.


\bibitem{OTFS1}
R. Hadani, S. Rakib, M. Tsatsanis, A. Monk, A. J. Goldsmith, A. F. Molisch, and R. Calderbank, ``Orthogonal Time Frequency Space Modulation,'' in \emph{IEEE Wireless Communications and Networking Conference (WCNC)}, San Francisco, CA, USA, March 2017.

\bibitem{OTFS2}
Z. Wei, W. Yuan, S. Li, J. Yuan, G. Bharatula, R. Hadani, and L. Hanzo, ``Orthogonal Time-Frequency Space Modulation: A Promising Next-Generation Waveform,'' \emph{IEEE Wireless Communications}, vol. 28, no. 4, pp. 136-144, August 2021.

\bibitem{OTFS3}
M. K. Ramachandran and A. Chockalingam, ``MIMO-OTFS in high-Doppler fading channels: Signal detection and channel estimation,'' in \emph{IEEE Global Communications Conference (GLOBECOM)}, Abu Dhabi, United Arab Emirates, December 2018.

\bibitem{OTFS4}
Shuangyang Li, Jinhong Yuan, Weijie Yuan, Zhiqiang Wei, Baoming Bai, and Derrick Wing Kwan Ng, "Performance Analysis of Coded OTFS Systems Over High-Mobility Channels," \emph{IEEE Transactions on Wireless Communications}, vol. 20, no. 9, pp. 6033-6048, April 2021.
\bibitem{OTFS5}
R. Hadani, S. Rakib, A. F. Molisch, C. Ibars, A. Monk, M. Tsatsanis, J. Delfeld, A. Goldsmith, and R. Calderbank, ``Orthogonal Time Frequency Space (OTFS) modulation for millimeter-wave communications systems,'' in \emph{IEEE MTT-S International Microwave Symposium (IMS)}, Honolulu, HI, USA, June 2017.
\bibitem{OTFS_dete}
Weijie Yuan, Zhiqiang Wei, Jinhong Yuan, and Derrick Wing Kwan Ng, ``A Simple Variational Bayes Detector for Orthogonal Time Frequency Space (OTFS) Modulation,'' \emph{IEEE Transactions on Vehicular Technology}, vol. 69, no. 7, pp. 7976-7980, April 2020.
\bibitem{eFF1}
Changyoung An and Heung-Gyoon Ryu, ``Design and Performance Evaluation of Spectral Efficient Orthogonal Time Frequency Space System,'' in \emph{2019 IEEE 2nd 5G World Forum (5GWF)}, Dresden, Germany, September 2019.
\bibitem{CSI_1}
Ziyi Huang, Shuai Cao, Hua Wei, and Li Li, ``Research on Channel Estimation Algorithm Based on OTFS System,'' in \emph{IEEE 6th Information Technology and Mechatronics Engineering Conference (ITOEC)}, Chongqing, China, March 2022.

\bibitem{CSI1}
M. Kollengode Ramachandran and A. Chockalingam, ``MIMO-OTFS in High-Doppler Fading Channels: Signal Detection and Channel Estimation,'' in \emph{IEEE Global Communications Conference (GLOBECOM)}, Abu Dhabi, United Arab Emirates, December 2018.


\bibitem{CSI2}
M. Kollengode Ramachandran and A. Chockalingam, ``MIMO-OTFS in High-Doppler Fading Channels: Signal Detection and Channel Estimation,'' in \emph{IEEE Global Communications Conference (GLOBECOM)}, Abu Dhabi, United Arab Emirates, December 2018.

\bibitem{CSI3}
Alexander Fish, Shamgar Gurevich, Ronny Hadani, Akbar M. Sayeed, and Oded Schwartz, ``Delay-Doppler Channel Estimation in Almost Linear Complexity,''\emph{IEEE Transactions on Information Theory}, vol. 59, no. 11, pp. 7632-7644, July 2013.


\bibitem{CSI_2}
Wenqian Shen, Linglong Dai, Jianping An, Pingzhi Fan, and Robert W. Heath, ``Channel Estimation for Orthogonal Time Frequency Space (OTFS) Massive MIMO,''\emph{IEEE Transactions on Signal Processing}, vol. 67, no. 16, pp. 4204-4217, August 2019.

\bibitem{CSI4}
P. Raviteja, Khoa T. Phan, and Yi Hong, ``Embedded Pilot-Aided Channel Estimation for OTFS in Delay–Doppler Channels,''\emph{IEEE Transactions on Vehicular Technology}, vol. 68, no. 5, pp. 4906-4917, March 2019.

\bibitem{CSI6}
Lei Zhao, Wen-Jing Gao, and Wenbin Guo, ``Sparse Bayesian Learning of Delay-Doppler Channel for OTFS System,''\emph{IEEE Communications Letters}, vol. 24, no. 12, pp. 2766-2769, June 2020.

\bibitem{CSI7}
Zhiqiang Wei, Weijie Yuan, Shuangyang Li, Jinhong Yuan, and Derrick Wing Kwan Ng, ``A New Off-grid Channel Estimation Method with Sparse Bayesian Learning for OTFS Systems,''in \emph{IEEE Global Communications Conference (GLOBECOM)}, 2021.

\bibitem{motivation1}
Sendy Phang, Michel T. Ivrlač, Gabriele Gradoni, Stephen C. Creagh, Gregor Tanner, and Josef A. Nossek, ``Near-Field MIMO Communication Links,''\emph{IEEE Transactions on Circuits and Systems I: Regular Papers}, vol. 65, no. 9, pp. 3027-3036, February 2018.

\bibitem{motivation2}
M. A. Nikravan, Do-Hoon Kwon, Hans G. Schantz, and Alfred H. Unden, ``Near-field MIMO communication utilizing both electric and magnetic field components,'' in \emph{IEEE Antennas and Propagation Society International Symposium (APSURSI)}, Memphis, TN, USA, July 2014.
\bibitem{motivation3}
A. E. Ampoma, G. Wen, Y. Huang, K. O. Gyasi, P. I. Tebe, and K. Ntiamoah-Sarpong, ``Spatial Correlation Models of Large-Scale Antenna Topologies Using Maximum Power of Offset Distribution and its Application,'' \emph{IEEE Access}, vol. 6, pp. 36295-36304, June 2018.
\bibitem{motivation4}
J.-q. Chen, Z. Zhang, T. Tang, and Y.-z. Huang, ``A non-stationary channel model for 5G massive MIMO systems,'' \emph{Frontiers of Information Technology \& Electronic Engineering}, vol. 18, no. 12, pp. 2101--2110, December 2017.

\bibitem{mMIMO3}
L. Lu, G. Y. Li, A. L. Swindlehurst, A. Ashikhmin, and R. Zhang, ``An Overview of Massive MIMO: Benefits and Challenges,'' in \emph{IEEE Journal of Selected Topics in Signal Processing}, vol. 8, no. 5, pp. 742-758, October 2014.

\bibitem{R13}
T. Zemen and D. L\"{o}schenbrand, ``Combating massive MIMO channel aging by orthogonal precoding,'' in \emph{IEEE 2nd 5G World Forum (5GWF)}, pp. 97--101, Dresden, Germany, September 2019.
\bibitem{R12}
L. Gaudio, G. Colavolpe, and G. Caire, ``OTFS vs. OFDM in the Presence of Sparsity: A Fair Comparison,'' \emph{IEEE Transactions on Wireless Communications}, vol. 21, no. 6, pp. 4410--4423, December 2021.
\bibitem{R11}
M. Mohammadi, H. Q. Ngo, and M. Matthaiou, ``Cell-Free Massive MIMO Meets OTFS Modulation,'' \emph{IEEE Transactions on Communications}, vol. 70, no. 11, pp. 7728-7747, September 2022.
\bibitem{R10}
H. Zhang, X. Huang, and J. A. Zhang, ``Comparison of OTFS diversity performance over slow and fast fading channels,'' in \emph{IEEE/CIC International Conference on Communications in China (ICCC)}, Changchun, China, August 2019.
\bibitem{DSS_OTFS}
J. Sun, Z. Wang, and Q. Huang, ``An Orthogonal Time Frequency Space Direct Sequence Modulation Scheme,'' in \emph{IEEE International Conference on Communications Workshops (ICC Workshops)}, Montreal, QC, Canada, June 2021.
\bibitem{mMIMO1}
A. Alkhateeb, G. Leus, and R. W. Heath, ``Limited Feedback Hybrid Precoding for Multi-User Millimeter Wave Systems,'' \emph{IEEE Transactions on Wireless Communications}, vol. 14, no. 11, pp. 6481-6494, July 2015.
\bibitem{mMIMO2}
L. G. Ord\'{o}\~{n}ez, D. P. Palomar, and J. R. Fonollosa, ``Fundamental diversity, multiplexing, and array gain tradeoff under different MIMO channel models,'' in \emph{IEEE International Conference on Acoustics, Speech and Signal Processing (ICASSP)}, Prague, Czech Republic, May 2011.

\bibitem{9557830}
W. Yuan, Z. Wei, S. Li, J. Yuan, and D. W. K. Ng, ``Integrated Sensing and Communication-Assisted Orthogonal Time Frequency Space Transmission for Vehicular Networks,'' \emph{IEEE Journal of Selected Topics in Signal Processing}, vol. 15, no. 6, pp. 1515-1528, October 2021. 

\bibitem{213131}
Z. Ling, Y. Wu, G. Zhang, and S. Sun, ``Integrated Sensing and Communications with OTFS: Application in V2I Communications,'' in \emph{Signal and Information Processing, Networking and Computers}, Singapore, February 2023.

\bibitem{9903393}
W. Yuan, Z. Wei, S. Li, R. Schober, and G. Caire, ``Orthogonal Time Frequency Space Modulation—Part III: ISAC and Potential Applications," \emph{IEEE Communications Letters}, vol. 27, no. 1, pp. 14-18, September 2023.
\bibitem{10152009}
W. Yuan, S. Li, Z. Wei, Y. Cui, J. Jiang, H. Zhang, and P. Fan, ``New Delay Doppler Communication Paradigm in 6G Era: A Survey of Orthogonal Time Frequency Space (OTFS),'' \emph{China Communications}, vol. 20, no. 6, pp. 1-25, June 2023. 
\bibitem{10164102}
Z. Tang, J. Jiang, W. Pan, and L. Zeng, ``The Estimation Method of Sensing Parameters Based on OTFS,'' \emph{IEEE Access}, vol. 11, no. 0, pp. 66035-66049, June 2023.
\bibitem{10051983}
A. S. Bondre and C. D. Richmond, ``On the Zak Transform-based Interpretation of OTFS Modulation,'' in \emph{Asilomar Conference on Signals, Systems, and Computers}, Pacific Grove, CA, USA, 2022.

%$
\bibitem{10095505}
A. S. Bondre, C. D. Richmond, A. Alkhateeb, and N. Michelusi, ``Sparse Delay-Doppler Channel Estimation for OTFS Modulation Using 2D-Music,'' in \emph{IEEE International Conference on Acoustics, Speech and Signal Processing (ICASSP)}, Rhodes Island, Greece, June 2023.

\bibitem{8647704}
A. Nimr, M. Chafii, M. Matthe, and G. Fettweis, ``Extended GFDM Framework: OTFS and GFDM Comparison,'' in \emph{IEEE Global Communications Conference (GLOBECOM)}, Abu Dhabi, United Arab Emirates, December 2018.

\bibitem{9737331}
A. Pfadler, T. Szollmann, P. Jung, and S. Stanczak, ``Leakage Suppression in Pulse-Shaped OTFS Delay-Doppler-Pilot Channel Estimation,'' \emph{IEEE Wireless Communications Letters}, vol. 11, no. 6, pp. 1181-1185, 2022.

\bibitem{9737044}
P. Zhu, X. Yin, J. Rodríguez-Pineiro, Z. Chen, P. Wang, and G. Li, ``Measurement-Based Wideband Space-Time Channel Models for 77GHz Automotive Radar in Underground Parking Lots,'' \emph{IEEE Transactions on Intelligent Transportation Systems}, vol. 23, no. 10, pp. 19105-19120, March 2022.

\bibitem{9625452}
B. Li, Z. Bai, J. Guo, Y. Yang, M. Yan, and X. Hao, ``Generalized Spatial Modulation based Orthogonal Time Frequency Space System,'' in \emph{IEEE 94th Vehicular Technology Conference (VTC2021-Fall)}, Norman, OK, USA, September 2021.
%%%
 
\bibitem{9538891}
S. Li, W. Yuan, Z. Wei, R. He, B. Ai, B. Bai, and J. Yuan, ``A Tutorial to Orthogonal Time Frequency Space Modulation for Future Wireless Communications,'' in \emph{IEEE/CIC International Conference on Communications in China (ICCC Workshops)}, Xiamen, China, July 2021.

\bibitem{9417451}
T. Thaj and E. Viterbo, ``Orthogonal Time Sequency Multiplexing Modulation,'' in \emph{IEEE Wireless Communications and Networking Conference (WCNC)}, Nanjing, China, May 2021.

\bibitem{9904495}
H. Liu, Y. Liu, M. Yang, and Q. Zhang, ``On the Characterizations of OTFS Modulation Over Multipath Rapid Fading Channel,'' \emph{IEEE Transactions on Wireless Communications}, vol. 22, no. 3, pp. 2008-2021, September 2023.

\bibitem{8892482}
P. Raviteja, Y. Hong, E. Viterbo, and E. Biglieri, ``Effective Diversity of OTFS Modulation,'' \emph{IEEE Wireless Communications Letters}, vol. 9, no. 2, pp. 249-253, November 2020.

\bibitem{9896669}
X. Li, H. Wang, X. Shen, Y. Ge, and Y. Lei, ``Delay-Doppler Reversal for OTFS System in Doubly-selective Fading Channels,'' in \emph{IEEE/CIC International Conference on Communications in China (ICCC Workshops)}, Sanshui, Foshan, China, August 2022.

\bibitem{8108396}
G. Berardinelli, K. Pedersen, F. Frederiksen, T. B. Sorensen, and P. Mogensen, ``Unique Word DFT-Spread-OFDM for Fast Time-Varying Channels,'' in \emph{IEEE 85th Vehicular Technology Conference (VTC Spring)}, Sydney, NSW, Australia, June 2017.

\bibitem{10056866}
Y. Ma, G. Ma, B. Ai, D. Fei, N. Wang, Z. Zhong, and J. Yuan, ``Characteristics of Channel Spreading Function and Performance of OTFS in High-Speed Railway,'' \emph{IEEE Transactions on Wireless Communications},, vol. 22, no. 10, pp. 7038-7054, October 2023.
%%%$

\bibitem{10038836}
W. Yuan, Z. Wei, J. Jiang, S. Zhang, J. Yuan, and P. Fan, ``Guest editorial: Orthogonal time frequency space modulation in 6G era,'' \emph{China Communications}, vol. 20, no. 1, pp. iii-vi, January 2023.

\bibitem{10001406}
H. Lin and J. Yuan, ``On Delay-Doppler Plane Orthogonal Pulse,'' in \emph{IEEE Global Communications Conference},  Rio de Janeiro, Brazil, December 2022, pp. 5589-5594.

\bibitem{10000697}
C. Shen, J. Yuan, Y. Xie, and H. Lin, ``Delay-Doppler Domain Estimation of Doubly-Selective Channels in Single-Carrier Systems,'' in \emph{IEEE Global Communications Conference}, Rio de Janeiro, Brazil, December 2022, pp. 5941-5946.

\bibitem{9625231}
G. Guo, Z. Jin, X. Zhang, and J. Wei, ``Joint Iterative Channel Estimation and Symbol Detection for Orthogonal Time Frequency Space Modulation,'' in \emph{IEEE 94th Vehicular Technology Conference (VTC2021-Fall)}, Norman, OK, USA, September 2021.

\bibitem{9745430}
D. Wang, B. Sun, F. Wang, X. Li, P. Yuan, and D. Jiang, ``Transmit diversity scheme design for rectangular pulse shaping based OTFS,'' \emph{China Communications}, vol. 19, no. 3, pp. 116-128, March 2022.

\bibitem{8424569}
P. Raviteja, K. T. Phan, Y. Hong, E. Viterbo, ``Interference Cancellation and Iterative Detection for Orthogonal Time Frequency Space Modulation,'' \emph{IEEE Transactions on Wireless Communications}, vol. 17, no. 10, pp. 6501-6515, August 2018.

\bibitem{8503182}
K. R. Murali and A. Chockalingam, ``On OTFS Modulation for High-Doppler Fading Channels,'' in \emph{Information Theory and Applications Workshop (ITA)},  San Diego, CA, USA, February 2018.

\bibitem{8686339}
G. D. Surabhi, R. M. Augustine, A. Chockalingam, ``On the Diversity of Uncoded OTFS Modulation in Doubly-Dispersive Channels,'' \emph{IEEE Transactions on Wireless Communications}, vol. 18, no. 6, pp. 3049-3063, April 2019.

\bibitem{8647394}
M. Kollengode Ramachandran and A. Chockalingam, ``MIMO-OTFS in High-Doppler Fading Channels: Signal Detection and Channel Estimation,'' in \emph{IEEE Global Communications Conference (GLOBECOM)}, Abu Dhabi, United Arab Emirates, December 2018.

\bibitem{10012421}
Z. Wei, H. Qu, Y. Wang, X. Yuan, H. Wu, Y. Du, K. Han, N. Zhang, and Z. Feng, ``Integrated Sensing and Communication Signals Toward 5G-A and 6G: A Survey,'' \emph{IEEE Internet of Things Journal}, vol. 10, no. 13, pp. 11068-11092, January 2023.

\bibitem{10164102}
Z. Tang, Z. Jiang, W. Pan, and L. Zeng, ``The Estimation Method of Sensing Parameters Based on OTFS,'' \emph{IEEE Access}, vol. 11, pp. 66035-66049, January 2023.
%%%^
\bibitem{9420020}
W. Yuan, S. Li, Z. Wei, J. Yuan, and D. W. K. Ng, ``Bypassing Channel Estimation for OTFS Transmission: An Integrated Sensing and Communication Solution,'' in \emph{IEEE Wireless Communications and Networking Conference Workshops (WCNCW)}, Nanjing, China, March 2021.

\bibitem{9747626}
S. Li, W. Yuan, J. Yuan, and G. Caire, ``On the Potential of Spatially-Spread Orthogonal Time Frequency Space Modulation for ISAC Transmissions,'' in \emph{IEEE International Conference on Acoustics, Speech and Signal Processing (ICASSP)}, Singapore, Singapore, May 2022.

\bibitem{RIS_OTFS1}
A. S. Bora, K. T. Phan, and Y. Hong, ``IRS-Assisted High Mobility Communications Using OTFS Modulation,'' \emph{IEEE Wireless Communications Letters}, vol. 12, no. 2, pp. 376-380, December 2023.

\bibitem{RIS1}
Q. Wu, S. Zhang, B. Zheng, C. You, and R. Zhang, ``Intelligent Reflecting Surface-Aided Wireless Communications: A Tutorial,'' \emph{IEEE Transactions on Communications}, vol. 69, no. 5, pp. 3313-3351, January 2021.

\bibitem{RIS_OTFS2}
C. Xu, L. Xiang, J. An, C. Dong, S. Sugiura, R. G. Maunder, L.-L. Yang, and L. Hanzo, ``OTFS-Aided RIS-Assisted SAGIN Systems Outperform Their OFDM Counterparts in Doubly Selective High-Doppler Scenarios,'' \emph{IEEE Internet of Things Journal}, vol. 10, no. 1, pp. 682-703, September 2023.

\bibitem{RIS_OTFS3}
Z. Huang, B. Zheng, and R. Zhang, ``Transforming Fading Channel From Fast to Slow: Intelligent Refracting Surface Aided High-Mobility Communication,'' \emph{IEEE Transactions on Wireless Communications}, vol. 21, no. 7, pp. 4989-5003, December 2022.

%%^^^%%%
\bibitem{RIS_OTFS4}
C. Xu, J. An, T. Bai, L. Xiang, S. Sugiura, R. G. Maunder, L.-L. Yang, and L. Hanzo, ``Reconfigurable Intelligent Surface Assisted Multi-Carrier Wireless Systems for Doubly Selective High-Mobility Ricean Channels,'' \emph{IEEE Transactions on Vehicular Technology}, vol. 71, no. 4, pp. 4023-4041, February 2022.

\bibitem{UAV1}
J. Mu, R. Zhang, Y. Cui, N. Gao, and X. Jing, ``UAV Meets Integrated Sensing and Communication: Challenges and Future Directions,'' \emph{IEEE Communications Magazine}, vol. 61, no. 5, pp. 62-67, May 2023.

\bibitem{UAV2}
I. Orikumhi, J. Bae, and S. Kim, ``UAV-Assisted Integrated Sensing and Communications for User Blockage Prediction,'' in \emph{International Conference on Information and Communication Technology Convergence (ICTC)}, Jeju Island, Korea, Republic of, October 2022, pp. 471-473.

\bibitem{PA1}
D.-T. Phan-Huy, M. Sternad, and T. Svensson, ``Adaptive large MISO downlink with Predictor Antenna array for very fast moving vehicles,'' in \emph{2013 International Conference on Connected Vehicles and Expo (ICCVE)}, Las Vegas, NV, USA, December  2013.

\bibitem{PA2}
H. Guo, B. Makki, M.-S. Alouini, and T. Svensson, ``Power Allocation in HARQ-Based Predictor Antenna Systems,'' \emph{IEEE Wireless Communications Letters}, vol. 9, no. 12, pp. 2025-2029, December 2020.

\bibitem{OFDM1}
B. Farhang-Boroujeny, ``OFDM Versus Filter Bank Multicarrier,'' \emph{IEEE Signal Processing Magazine}, vol. 28, no. 3, pp. 92-112, April 2011.

\bibitem{OFDM2}
T. Hwang, C. Yang, G. Wu, S. Li, and G. Y. Li, ``OFDM and Its Wireless Applications: A Survey,'' \emph{IEEE Transactions on Vehicular Technology}, vol. 58, no. 4, pp. 1673-1694, August 2009.

\bibitem{mmwave1}
S. A. Busari, K. M. S. Huq, S. Mumtaz, L. Dai, and J. Rodriguez, ``Millimeter-Wave Massive MIMO Communication for Future Wireless Systems: A Survey,'' \emph{IEEE Communications Surveys & Tutorials}, vol. 20, no. 2, pp. 836-869, December 2018.

%%%%%%%%%%
\bibitem{SDR_OTFS}
P. Karpovich, T. P. Zielinski, R. Maksymiuk, K. Abratkiewicz, P. Tomikowski, and P. Samczyński, ``Experimental Testing of an OTFS-Modulated Waveform in a Joint Radar-Comm System,'' in \emph{2023 IEEE Radar Conference (RadarConf23)}, 2023, pp. 1-6.

\bibitem{R9}
M. F. Keskin, H. Wymeersch, and A. Alvarado, ``Radar Sensing with OTFS: Embracing ISI and ICI to Surpass the Ambiguity Barrier,'' in \emph{2021 IEEE International Conference on Communications Workshops (ICC Workshops)}, 2021, pp. 1-6.

\bibitem{R8}
H. Zhang, X. Huang, and J. A. Zhang, ``Comparison of OTFS Diversity Performance over Slow and Fast Fading Channels,'' in \emph{2019 IEEE/CIC International Conference on Communications in China (ICCC)}, 2019, pp. 828-833.

\bibitem{R8}
Z. Yuan, K. Niu, and C. Dong, ``Channel Prediction and PMI/RI Selection in MIMO-OFDM Systems Based on Deep Learning,'' in \emph{2021 IEEE 32nd Annual International Symposium on Personal, Indoor and Mobile Radio Communications (PIMRC)}, 2021, pp. 598-603.

\bibitem{R7}
K. E. Baddour and N. C. Beaulieu, ``Autoregressive modeling for fading channel simulation,'' \emph{IEEE Transactions on Wireless Communications}, vol. 4, no. 4, pp. 1650-1662, 2005.

\bibitem{R6}
N. Beigiparast, G. M. Guvensen, and E. Ayanoglu, ``Spatial Correlation in Single-Carrier Massive MIMO Systems,'' in \emph{Information Theory and Applications Workshop (ITA)}, San Diego, CA, USA, February 2020.

\bibitem{aging1}
T. Younas, M. Mekonnen, G. Farid, S. Tahir, O. Younas, W. A. Wattoo, M. Farhan, and M. Liaqat, ``Investigation of LS-MIMO systems with channel aging effects,'' \emph{Physical Communication}, vol. 40, p. 101088, June 2020.

\bibitem{OTFS_effective}
L. Gaudio, M. Kobayashi, G. Caire, and G. Colavolpe, ``On the Effectiveness of OTFS for Joint Radar Parameter Estimation and Communication,'' \emph{IEEE Transactions on Wireless Communications}, vol. 19, no. 9, pp. 5951-5965, June 2020.

\bibitem{mMIMOradar}
C. Kai, X. Zhang, X. Hu, and W. Huang, ``Joint pilot design and beamforming optimization in massive MIMO surveillance systems,'' \emph{China Communications}, vol. 19, no. 4, pp. 83-97, April 2022.

\bibitem{temporal}
K. T. Truong and R. W. Heath, ``Effects of channel aging in massive MIMO systems,'' \emph{Journal of Communications and Networks}, vol. 15, no. 4, pp. 338-351, August 2013.
%%
\bibitem{PA3}
D.-T. Phan-Huy and M. Helard, ``Large MISO beamforming for high speed vehicles using separate receive \& training antennas,'' in \emph{IEEE 5th International Symposium on Wireless Vehicular Communications (WiVeC)}, Dresden, Germany, June 2013.

\bibitem{work1}
S. K. Dehkordi, L. Gaudio, M. Kobayashi, G. Colavolpe, and G. Caire, ``Beam-Space MIMO Radar with OTFS Modulation for Integrated Sensing and Communications,'' in \emph{IEEE International Conference on Communications Workshops (ICC Workshops)}, Seoul, Korea, Republic of, May 2022, pp. 509-514.

\bibitem{work2}
P. Karpovich and T. P. Zielinski, ``Random-Padded OTFS Modulation for Joint Communication and Radar/Sensing Systems,'' in \emph{23rd International Radar Symposium (IRS)}, Gdansk, Poland, September 2022, pp. 104-109.

\bibitem{work3}
H. Zhang, T. Zhang, and Y. Shen, ``Modulation Symbol Cancellation for OTFS-Based Joint Radar and Communication,'' in \emph{IEEE International Conference on Communications Workshops (ICC Workshops)}, Montreal, QC, Canada, June 2021.

\bibitem{work4}
L. Gaudio, M. Kobayashi, G. Caire, and G. Colavolpe, ``On the Effectiveness of OTFS for Joint Radar Parameter Estimation and Communication,'' \emph{IEEE Transactions on Wireless Communications}, vol. 19, no. 9, pp. 5951-5965, June 2020.

\bibitem{work5}
O. Zacharia and M. Vani Devi, ``Fractional Delay and Doppler Estimation for OTFS Based ISAC Systems,'' in \emph{IEEE Wireless Communications and Networking Conference (WCNC)}, Glasgow, United Kingdom, March 2023.

\bibitem{work6}
S. P. Muppaneni, S. R. Mattu, and A. Chockalingam, ``Channel and Radar Parameter Estimation With Fractional Delay-Doppler Using OTFS,'' \emph{IEEE Communications Letters}, vol. 27, no. 5, pp. 1392-1396, March 2023.

\bibitem{work7}
Z. Cui, J. Hu, J. Cheng, and G. Li, ``Multi-Domain NOMA for ISAC: Utilizing the DOF in the Delay-Doppler Domain,'' \emph{IEEE Communications Letters}, vol. 27, no. 2, pp. 726-730, December 2023.

\bibitem{work8}
K. Wu, J. A. Zhang, X. Huang, and Y. J. Guo, ``OTFS-Based Joint Communication and Sensing for Future Industrial IoT,'' \emph{IEEE Internet of Things Journal}, vol. 10, no. 3, pp. 1973-1989, December 2023.

\bibitem{work9}
B. Wang, N. Li, Z. Jiang, J. Zhu, X. She, and P. Chen, ``On Performance Evaluation of OTFS and OFDM Modulations for Sensing,'' in \emph{14th International Conference on Wireless Communications and Signal Processing (WCSP)}, Nanjing, China, November 2022, pp. 427-431.

\bibitem{work10}
A. Correas-Serrano, N. Petrov, M. Gonzalez-Huici, and A. Yarovoy, ``Comparison of Radar Receivers for OFDM and OTFS waveforms,'' in \emph{19th European Radar Conference (EuRAD)}, Milan, Italy, September  2022.

\bibitem{work11}
S. E. Zegrar, S. Rafique, and H. Arslan, ``OTFS-FMCW Waveform Design for Low Complexity Joint Sensing and Communication,'' in \emph{IEEE 33rd Annual International Symposium on Personal, Indoor and Mobile Radio Communications (PIMRC)}, Kyoto, Japan, September 2022.

\bibitem{work12}
S. Li, W. Yuan, W. Yuan, G. Caire, ``On the Potential of Spatially-Spread Orthogonal Time Frequency Space Modulation for ISAC Transmissions,'' in \emph{IEEE International Conference on Acoustics, Speech and Signal Processing (ICASSP)}, 2022, pp. 8722-8726.

\bibitem{work13}
Y. Wu, C. Han, and Z. Chen, ``An Energy-Efficient DFT-Spread Orthogonal Time Frequency Space System for Terahertz Integrated Sensing and Communication,'' in \emph{IEEE International Conference on Communications},  Seoul, Korea, Republic of, May 2022.

\bibitem{10068080}
M. Ubadah and S. Khan Mohammed, ``Impact of Sinusoidal Co-channel CW Interference on the Spectral Efficiency of OTFS Modulation,'' in \emph{National Conference on Communications (NCC)}, Guwahati, India, February 2023.

\bibitem{9919200}
V. S. Bhat, G. Harshavardhan, and A. Chockalingam, ``Input-Output Relation and Performance of RIS-Aided OTFS With Fractional Delay-Doppler,'' \emph{IEEE Communications Letters}, vol. 27, no. 1, pp. 337-341, October 2023.
 

\bibitem{9473535}
A. Pfadler, P. Jung, T. Szollmann, and S. Stanczak, ``Pulse-Shaped OTFS over Doubly-Dispersive Channels: One-Tap vs. Full LMMSE Equalizers,'' in \emph{IEEE International Conference on Communications Workshops (ICC Workshops)}, Montreal, QC, Canada, June  2021.



\end{thebibliography}

